Diagonally non-computable functions and fireworks

A set C of reals is said to be negligible if there is no probabilistic algorithm which generates a member of C with positive probability. Various classes have been proven to be negligible, for example the Turing upper-cone of a non-computable real, the class of coherent completions of Peano Arithmetic or the class of reals of minimal degrees. One class of particular interest in the study of negligibility is the class of diagonally non-computable (DNC) functions, proven by Kucera to be non-negligible in a strong sense: every Martin-L\"of random real computes a DNC function. Ambos-Spies et al. showed that the converse does not hold: there are DNC functions which compute no Martin-L\"of random real. In this paper, we show that such the set of such DNC functions is in fact non-negligible. More precisely, we prove that for every sufficiently fast-growing computable~$h$, every 2-random real computes an $h$-bounded DNC function which computes no Martin-L\"of random real. Further, we show that the same holds for the set of reals which compute a DNC function but no bounded DNC function. The proofs of these results use a combination of a technique due to Kautz (which, following a metaphor of Shen, we like to call a `fireworks argument') and bushy tree forcing, which is the canonical forcing notion used in the study of DNC functions.

==> existsk_dnrk.tex <==


\begin{theorem}\label{thm:existsk-dnrk-wwkl}
$\rca + \bst \not \vdash (\exists k)(\forall f)\dnr(k,f) \imp \wwkl$
\end{theorem}


\subsection{Proof sketch of Theorem~\ref{thm:existsk-dnrk-wwkl}}

Similar to Theorem~\ref{thm:main-theorem},
we will construct a DNC function $f$ within a very fast-growing tree
and ensure that for every functional $\Gamma$,
either $\Gamma^f$ is not total or it has initial segment of high randomness
deficiency.

For any standard $k$, any $k$-bounded DNC function computes a set of PA degree
and in particular a Martin-Löf random. Moreover the proof is formalizable
over $\rca$. Then if $f$ is a $k$-bounded proper DNC function, then
must be non-standard. In order to build such a function, we will place ourself 
in a model $\Mcal = (\Nb, \Scal)$ of $\rca + \bst + \neg \ist$. A well-known result of proof theory states
that for every such model, there exists a $\Sigma^0_2$ definable proper cut $I$ -- i.e. a downward and successor-closed 
proper subset of $\Nb$ -- together with an increasing $\Delta^0_2$ cofinal function $c : I \to \Nb$.

The construction will be made by stages $s \in I$. 
As in previous proof, we will have at each stage $i$ a tree $T_i$ very fast-growing for some function $h$
which is $h_i$-bushy above $\sigma_i$. Before giving the construction
we will detail some tricky points raised by the new constraint of 
building a $k$-bounded proper DNC function.

\smallskip

\emph{Forcing $f$ to have a bounded range.}
In previous proof, we ensured $f$ to be $h$-bounded by starting the construction
with the full tree $h^{<\omega}$. However we want now $f$ to have a range bounded by some $k$.
This is why $h_0$ will be very fast-growing from the point of view
of $I$, but not of $\Nb$. More precisely, for any function $h$, we can define the function $h^{*}$
by fixing a $k \in \Nb \setminus I$ and setting $h^{*}(i) = h(i)$ if $i < k$, and $h^{*}(i) = h(k)$ otherwise.
Then taking $h_0 = h^{*}$ we obtain a $h(k)$-bounded function.

\smallskip

\emph{Forcing a non-standard deficiency.}
Another new difficulty lies in forcing the initial segments of a functional $\Gamma^f$
to have an arbitrarily large deficiency of randomness. By definition,
a set $X$ is Martin-Löf random if there is an $r \in \Nb$
such that $K(X \restr n) \geq n - r$ for every $n \in \Nb$.
In this case, $r$ can be non-standard and much larger than the $k$ making $f$ $k$-bounded
and we can only ask questions about $j$-smallness/bigness of events for $j << k$.
Hopefully Avigad \& al. proved in \cite{avigad2012algorithmic}
that having $\rca \vdash \ran{1} \biimp \wwkl$. Hence taking the tree
$T = \set{\sigma \in 2^{<\Nb} : K(\sigma) \geq n - 1}$ we are sure that
in any model of $\rca + \ran{1}$ there exists a set of randomness deficiency at most 1.
Hence it suffices to ensure that the deficiency of an initial segment of $\Gamma^f$
is at least 2.

\smallskip

\emph{Forcing deficiency and totality.}
We want our function $f$ to be total over $\Nb$, and this by stages $s \in I$.
A natural way consists of ensuring that at step $i$, the stem $\sigma_i$
of the tree $T_i$ has length at least $c(i)$. However this raises a problem
when trying to force initial segments of $\Gamma^f$ to have a high randomness deficiency.
We used to describe initial segments of $\Gamma^f$ given the description of current stage,
but at stage $i$, $\sigma_i$ has length at least $c(i)$ which may be much larger than $k$
and so we would have to describe an even larger initial segment of $\Gamma^f$ to have
some compression property. This is not possible for the same reasons as previous points,
i.e. we can only ask questions about $j$-smallness/bigness of events for $j << k$.
This is why we need first to construct a 4-uple $(\sigma, T, B, h, j)$
where $\sigma$ is a DNC string of bounded length, $T$ is a tree with no dead-ends
which is $h$-bushy above $\sigma$, $B$ is an upward-closed $\Sigma^0_1$ set 
$j$-small above $\sigma$ and $h, j$ are orders. We will ensure that any path in $T$
which avoids $B$ is a DNC which computes no Martin-Löf random. The second step consists of constructing a
path in this tree. This 4-uple is constructed by stages $s \in I$ but at each stage,
$\sigma_s$ has length $s$ and not $c(s)$ anymore. Thus the description of stage $s$ will remain short
and we will be able to compress information of large initial segments of $\Gamma^f$ 
without asking for too much convergence.
\ludovic{TODO: Does such a $\sigma$ exist ? Is the tree $T$ computable ?...
The problem is that $I$ is not computable, hence $T = \bigcap_{s \in I} T_s$ may not be.}

\smallskip

\emph{Diagonalizing against a non-standard number of functionals.}
Another subtlety when working with non-standard models is that we have to diagonalize
against a non-standard number of functionals, and this in a bounded number of stages.
Thus at each stage we will have to diagonalize against a block of functionals.
A way to do that would be to construct a function $\beta$ such that for each $e \in \Nb$,
if there is a $\Gamma^f_i$ which is Martin-Löf random for some $i < e$ then so is $\Gamma^f_{\beta(e)}$.
However such a function does not exist. But we can weaken our constraint by asking that
$\Gamma^f_{\beta(e)}(n)$ is a binary string of length $n$ for each $n$ and
if $\Gamma^f_i$ is MLR for some $i < e$, then $\Gamma^f_{\beta(e)}$ will \emph{eventually}
enumerate only initial segments of MLRs. Thus it will suffice to diagonalize against
$\Gamma^f_{\beta(e)}(n)$ for cofinally many $n$ and $e$.

\smallskip

\emph{Preserving $\bst$.}
Adding new sets may make fail $\bst$ in the new model. However
a well-known lemma states that if $g' \leq_T f'$ for some functions $g$ and $g$,
and $\bst$ holds relative to $f$, then $\bst$ holds relative to $g$.
Hence ensuring to add only low sets will make $\bst$ preserved.
The technic for deciding 
\ludovic{TODO: Explain how we force lowness}

\subsection{Formal proof}

Given a model $\Mcal$, we will distinguish $\omega$ which denotes the set of standard numbers
and $\Nb$ which is the first order part of $\Mcal$.

\begin{definition}
Given a constant $n \in \Nb$ and 
$\mlr(n,f)$ is the $\Pi^{0,f}_1$ class of Martin-Löf randoms relative to $f$ with deficiency $n$,
i.e. $\mlr(n,f) = \set{X \in 2^{<\Nb} : (\forall \sigma \prec X)K^f(\sigma) > \card{\sigma} - n}$.
By abuse of notation, $\mlr(n,f)$ is also considered as the statement $(\exists g)[g \in \mlr(n,f)]$.
$\ran{1}$ is the principle $(\forall f)(\exists n)\mlr(n,f)$.
\end{definition}

\begin{theorem}[Avigad \& al. in \cite{avigad2012algorithmic}]\label{thm:ran-wwkl}
$\rca \vdash \ran{1} \biimp \wwkl$
\end{theorem}

\begin{definition}
A string $\sigma$ is \emph{$n$-complex} if $(\forall \tau \preceq \sigma)(K(\tau) > \card{\tau} - n)$. 
A function $h : \Nb \to 2^{<\Nb}$ is \emph{$n$-complex} if
for every $l \in \Nb$, $\card{h(l)} = l$ and $h(l)$ is an $n$-complex string.
$h$ is \emph{eventually $n$-complex} if the number of $l$ such that $h(l)$ is not $n$-complex is bounded.
\end{definition}

If $h$ is $n$-complex and $m > n$ then $h$ is also $m$-complex.
Theorem~\ref{thm:ran-wwkl} states that it suffices to diagonalize against 1-complex
functions to ensure that we do not get a model of $\ran{1}$ as we see in Lemma~\ref{lem:ran-complex}.

\begin{lemma}\label{lem:ran-complex}
$\rca \vdash \ran{1} \imp (\exists h)(h \mbox{ is 1-complex})$
\end{lemma}
\begin{proof}
Consider the $f$-computable tree $T = \set{\sigma \in 2^{<\Nb} : K(\sigma) > \card{\sigma} - 1}$.
By Theorem-\ref{thm:ran-wwkl} there exists a path $X \in [T]$.
Then the function $h$ which to $n$ associates the initial segment of $X$ of length $n$
is 1-complex.
\end{proof}

Given a function $f$, define an $f$-computable function $\beta_f : \Nb \times \Nb \to \Nb$
so that for every $n, e \in \Nb$, $\beta_f(n, e)$ is an index for a program such that,
for every $l \in \Nb$ and function $g$, $\Phi^{f \oplus g}_{\beta_f(n,e)}(l)$
searches for a pair $\tuple{i,s}$ such that $l,i < s$, $\Phi^{f \oplus g}_{i,s}(l) \in 2^l$ 
and $\neg (\exists l_0 < l)(K_l(\Phi^{f \oplus g}_{j,l}(l_0)) \leq l_0 - n)$.
If such a pair is found, then $\Phi^{f \oplus g}_{\beta_f(n,e)}(l) = \Phi^{f \oplus g}_{i,s}(l)$.
Otherwise $\Phi^{f \oplus g}_{\beta_f(n,e)}(l) \uparrow$.

\begin{lemma}[$\rca$]\label{lem:n-complex-block}
Let $f$, $g$ be functions and $n, e \in \Nb$. If there is an $i < e$ such that
$\Phi^{f \oplus g}_i$ is $n$-complex then $\Phi^{f \oplus g}_{\beta_f(n,e)}$ is
eventually $n$-complex.
\end{lemma}
\begin{proof}
If $\Phi^{f \oplus g}_i$ is $n$-complex for some $i < e$ 
then $\Phi^{f \oplus g}_{\beta_f(n,e)}$ is total. 
The finite set $X = \set{k < e : \exists l, s : K_s(\Phi^{f \oplus g}_{j,s}(l)) \leq l - n}$
exists by bounded $\Sigma^0_1$-comprehension.
$\bsigs{1}$ then provides a bound $m$ such that 
$(\forall j \in X)(\exists l,s < m)(K_s(\Phi^{f \oplus g}_{j,s}(l)) \leq l - n)$.
We will show that $(\forall l > m)(K(\Phi^{f \oplus g}_{\beta_f(n,e)}(l)) > l - n)$.
Suppose for a contradiction that $l > m$ and $K(\Phi^{f \oplus g}_{\beta_f(n,e)}(l)) \leq l - n$.
By the definition of $\beta_f(n,e)$, there is a $j < e$ and an $s$ such that
$\Phi^{f \oplus g}_{\beta_f(n,e)}(l) = \Phi^{f \oplus g}_{j,s}(l)$
and $\neg (\exists l_0 < l)(K_l(\Phi^{f \oplus g}_{j,l}(l_0)) \leq l_0 - n)$.
By $K(\Phi^{f \oplus g}_{\beta_f(n,e)}(l)) \leq l - n$, there is a $t > s$ such that
$K_t(\Phi^{f \oplus g}_{j,t}(l)) \leq l - n$. Hence $j \in X$, hence there are
$l_0, s < m$ such that $K_s(\Phi^{f \oplus g}_{j,s}(l_0)) \leq l_0 - n$, but $m < l$,
so $(\exists l_0 < l)(K_l(\Phi^{f \oplus g}_{j,l}(l_0)) \leq l_0 - n)$, a contradiction.
\end{proof}

Putting Lemma~\ref{lem:ran-complex} and Lemma~\ref{lem:n-complex-block} together,
fix a cut $I \subseteq \Nb$ and a cofinal function $c : I \to \Nb$.
If $f \oplus g$ computes a MLR, there exists $n \in I$ such that
$\Phi^{f \oplus g}_{\beta_f(1, c(n))}$ is eventually 1-complex.

